Super Non-singular Decompositions of Polynomials and their Application to Robustly Learning Low-degree PTFs

We study the efficient learnability of low-degree polynomial threshold functions (PTFs) in the presence of a constant fraction of adversarial corruptions. Our main algorithmic result is a polynomial-time PAC learning algorithm for this concept class in the strong contamination model under the Gaussian distribution with error guarantee $O_{d, c}(\text{opt}^{1-c})$, for any desired constant $c>0$, where $\text{opt}$ is the fraction of corruptions. In the strong contamination model, an omniscient adversary can arbitrarily corrupt an $\text{opt}$-fraction of the data points and their labels. This model generalizes the malicious noise model and the adversarial label noise model. Prior to our work, known polynomial-time algorithms in this corruption model (or even in the weaker adversarial label noise model) achieved error $\tilde{O}_d(\text{opt}^{1/(d+1)})$, which deteriorates significantly as a function of the degree $d$. Our algorithm employs an iterative approach inspired by localization techniques previously used in the context of learning linear threshold functions. Specifically, we use a robust perceptron algorithm to compute a good partial classifier and then iterate on the unclassified points. In order to achieve this, we need to take a set defined by a number of polynomial inequalities and partition it into several well-behaved subsets. To this end, we develop new polynomial decomposition techniques that may be of independent interest.

==> figure.tex <==
      \definecolor{mycyan}{RGB}{42,161,152}
\definecolor{myred}{RGB}{220,50,47}
\begin{figure}
	\centering
	\begin{tikzpicture}[scale=1, every node/.style={transform shape} ]
	\coordinate (start) at (0.5,0.5);
	\coordinate (center) at (0,0);
	\coordinate (end) at (0,0.7);
	\coordinate (end2) at (-0.12/0.7634,0.366/0.7634);
	\coordinate (start2) at (0,0.7);
	\coordinate (start3) at (3,0);
	\coordinate (end3) at (45:3);
	\coordinate (start4) at (135:2);
	\coordinate (end4) at (-2,0);
	% \draw (0,0) circle (3);
	\draw[fill=mycyan, opacity=0.6] (0,0) -- (3,0) arc (0:45:3.0cm)--cycle;
 \draw[fill=mycyan, opacity=0.6] (0,0) -- (-2,0) arc (180:225:2.0cm)--cycle;
%  \begin{scope}[thin]
% \clip(0,1) rectangle (3,3);
% \draw[pattern=north west lines, pattern color=red, opacity=1] (0,0) -- (3,0) arc (0:45:3.0cm) -- cycle;
% \end{scope}

% 	\draw[fill=mycyan, opacity=0.6] (0,0) -- (-3,0) arc (180:225:3.0cm) -- cycle;
% 	 \begin{scope}[thin]
% \clip(0,-1) rectangle (-3,-3);
% \draw[pattern=north west lines, pattern color=red, opacity=1] (0,0) -- (-3,0) arc (180:225:3.0cm) -- cycle;
% \end{scope}
	\draw[black,thick,-] (-2,0) -- (3,0) ;
 	\draw[black,dashed,-] (-2,0.5) -- (3,0.5) ;
  	\draw[black,dashed,-] (-2,1) -- (3,1) ;
    	\draw[black,dashed,-] (-2,1.5) -- (3,1.5) ;

\draw[blue,thick,-] (0,0.5) -- (3,0.5) ;
     \draw[blue,thick,-] (0.5,0.5) -- (0.5,1) ;
      \draw[blue,thick,-] (0.5,1) -- (3,1) ;
     % \draw[black,thick,-] (0,-1) -- (0,2.5) ;
          \draw[blue,thick,-] (1,1) -- (1,1.5) ;
           \draw[blue,thick,-] (1,1.5) -- (3,1.5) ;
     \draw[black,thick,-] (0,-1) -- (0,2.5) ;
     \draw[blue,dashed,-] (1,1.5)--(1,0)  node[below ]{$\Theta(i)$};
	% \draw[->] (0,0) -- (3,0) node[anchor=north west,black] {$\vec e_1$};
	% \draw[->] (0,-1) -- (0,2.5) node[anchor=south east] {$\vec e_2$};
% \draw[purple,thick,-] (3.2*0.95,-3.2*0.95) -- (-3.2*0.95,3.2*0.95) node[anchor= south east] {};
	% \draw[yellow,thick,-] (-4.4*0.94,-1.2*0.94) -- (4.4*0.94,1.2*0.94) node[anchor= south east] {};
	\draw[black,thick,->] (0,-0) -- (-0.45,0.45) node[anchor= south ] {$\vec v^\ast$};
 \draw[black,thick,->] (0,-0) -- (0.5,0) node[anchor= south ] {$\vec u$};
	% \draw[purple,thick,->] (0,-0) -- (0.707,0.707)node[anchor= south east,above] {$\wt{\vec w}$};
 \draw[purple,thick,<->] (-2,0) -- (-2,0.5)node[anchor= south east,below left] {$\delta$};
\draw[purple,thick,<->] (-2,0.5) -- (-2,1)node[anchor= south east,below left] {$\delta$};
\draw[purple,thick,<->] (-2,1) -- (-2,1.5)node[anchor= south east,below left] {$\delta$};
 % \draw[purple,thick,<->] (2,0) -- (2,2.12)node[anchor= south east,right] {$ \sin\theta$};
 
	\draw[black] (-1,-1) -- (2,2);
	\draw[black,thick ,->] (0,0) -- (0,0.5) node[above right] {$\bw$};
\pic [draw, <->, angle radius=15mm, angle eccentricity=1.3, "$\theta = \Theta(\delta)$"] {angle = start3--center--end3};
	% \pic [draw, <->, angle radius=15mm, angle eccentricity=1.2, "$\theta_2$"] {angle = start4--center--end4};
% \node[] at (-2,-1.3) {$C$};
% \node[] at (2,1.3) {$C$};
% \draw[black,dashed ,-] (2*1.414*3/4,2*1.414*3/4) -- (4,2.12) node[above right] {};
	% \node[] at (2*1.414*3/4,2*1.414*3/4)[below] {$Z$};
\end{tikzpicture}
	\caption{The disagreement region between a halfspace with normal vector $\vec w$ and the target $\vec v^\ast$ is shown in green.
 The unit direction $\vec u$ corresponds to the projection of $\vec v^\ast$
 on the orthogonal complement of $\vec w$.
 We assume that the $\ell_2$ distance of the two halfspaces is $\delta$ (and thus their angle is $\Theta(\delta)$). Since the slabs $S_i = \{i \delta \leq |\vec x \cdot \vec w| \leq (i+1) \delta \}$ have width $\delta$, the $x$-coordinate of the start of the $i$-th box is $\Theta(i)$.
 }
	\label{fig:wedge}
\end{figure}

==> reasonable-Gaussian-backup.tex <==
\begin{claim} \label{eq:condition-norm-under-reasonable-gaussian}
Let $d, m, N \in \mathbb Z^+$.
Let $f:\R^m \mapsto \R$ be a degree-$d$ polynomial, and $\normal(\vec \mu, \vec \Sigma)$ be a $(\delta, N )$-reasonable Gaussian.
Let $\vec a \in \R^k$.
Define the restricted function $ f_{\vec a}: \R^{m-k} \mapsto \R$ as $ f_{\vec a}(\vec x) = f(\vec a, \vec x)$.
Let $\text{LC}(  f_{\vec a} )$ be the absolute value of the largest coefficient in $ f_{\vec a}$.
It holds
\begin{align}
\label{eq:conditional-expectation}
\poly_{d,m,N}(\log^{-1}(1/\delta))
\; \delta^{d} \; \text{LC}(  f_{\vec a} )
&\leq 
\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x_1 = \vec a_1, \cdots, \vec x_k = \vec a_k
\rp]  \\
&\leq \poly_{d,m,N}(\log(1/\delta)) \; \delta^{-d} \; \text{LC}(  f_{\vec a} ). 
\end{align}
\end{claim}
\begin{proof}
We first write down the block decomposition of $\vec \mu$ and $\vec \Sigma$:
\begin{align}
\vec \mu = \begin{bmatrix}
    &\vec \mu_1, \\
    &\vec \mu_2
\end{bmatrix}   \, , \,
\vec \Sigma = \begin{bmatrix}
    &\vec \Sigma_{1,1} &\vec \Sigma_{1,2} \\ 
    &\vec \Sigma_{2,1} &\vec \Sigma_{2,2}.
\end{bmatrix}
\end{align}
where $\mu_1 \in \R^k$ is the mean of the $k$ coordinates being conditioned, $\mu_2 \in \R^{m-k}$ is the mean of the rest of coordinates, and $\vec \Sigma_{1,1} \in \R^{k \times k}, \vec \Sigma_{1,2} \in \R^{k \times (m-k)}, \vec \Sigma_{2,1} \in \R^{k \times (m-k)}, \vec \Sigma_{2,2} \in \R^{(m-k) \times (m-k)}$ are the corresponding sub-covariance matrices.
Since $\sigma_{\min} \lp( \vec \Sigma \rp) > \delta$, the same holds for $\vec \Sigma_{2,2}$.
Notice that the distribution $\normal(\vec \mu, \vec \Sigma)$ under the conditioning is another $(m-k)$-dimensional Gaussiain distribution 
$\normal( \vec {\tilde \mu}, \vec {\tilde \Sigma} )$
with the parameters given by
\begin{align*}
&\vec {\tilde \mu} = \vec \mu_{1} + \vec \Sigma_{1,2} \; \vec \Sigma_{2,2}^{-1}  \; (\vec a - \vec \mu_2) \, , \\
&\vec {\tilde \Sigma}
= \vec \Sigma_{1,1} - 
\vec \Sigma_{1,2} 
\vec \Sigma_{2,2}^{-1} \vec \Sigma_{2,1}.
\end{align*}
We proceed to bound the parameters.
Since $\snorm{2}{\vec \mu} \leq \log^{N}(1/\delta) $ and
$ \delta \vec I \leq   \vec \Sigma  \leq \log^{N}(1/\delta)$, 
the entries in $\vec \mu_1$, $\vec \mu_2$, $\vec \Sigma_{1,1}$, $\vec \Sigma_{1,2}$, $\vec \Sigma_{2,1}$ are all upper bounded by $\log^{N}(1/\delta)$ and the entries in $\vec \Sigma_{2,2}^{-1}$ are upper bounded by $\delta^{-1}$.
It then follows that $\snorm{2}{ \tilde \mu } \leq 
O_{d,m}(1) \; \delta^{-1} \; \log^{2N}(1/\delta)$.
For $\vec {\tilde \Sigma}$, we remark its expression is exactly the Schur complement of $\vec \Sigma_{2,2}$ in $\vec \Sigma$.
Therefore, we can employ the following fact.
\begin{fact}
Let $\vec \Sigma \in \R^{m \times m}$.
Suppose \begin{align}
\vec \Sigma = \begin{bmatrix}
    &\vec \Sigma_{1,1} &\vec \Sigma_{1,2} \\ 
    &\vec \Sigma_{2,1} &\vec \Sigma_{2,2}.
\end{bmatrix}    
\end{align}
 where $\vec \Sigma_{1,1} \in \R^{k \times k}, \vec \Sigma_{1,2} \in \R^{k \times (m-k)}, \vec \Sigma_{2,1} \in \R^{k \times (m-k)}, \vec \Sigma_{2,2} \in \R^{(m-k) \times (m-k)}$.
 Denote $\vec S$ as the Schur complement $$
 \vec S
 = \vec \Sigma_{1,1} - 
\vec \Sigma_{1,2} 
\vec \Sigma_{2,2}^{-1} \vec \Sigma_{2,1}.
 $$
 If $\vec \Sigma$ is positive definite, then it holds
 $$
 \lambda_t( \vec \Sigma )
 \geq \lambda_t(\vec S)
 \geq \lambda_{t + k}(\vec \Sigma).
 $$
\end{fact}
This then gives us
$$
 \delta \vec I \leq \vec {\tilde \Sigma}
 \leq \log^N(1/\delta) \vec I.
$$

We are ready to bound the conditional expectation in \Cref{eq:conditional-expectation}.
Notice that
$$
\E_{ \vec y \sim \normal( \vec {\tilde \mu}, \vec {\tilde \Sigma} ) }
\lp[
f_{\vec a}(\vec y)
\rp]
=
\E_{ \vec y \sim \normal( \vec 0, \vec I) }
\lp[
f_{\vec a}\lp( {\vec {\tilde \Sigma} }^{1/2} \lp(\vec y - \vec {\tilde \mu}\rp)\rp)
\rp].
$$
% Define $\vec q_{\vec a}: \R^m \mapsto \R$ as $\vec q_{\vec a}(\vec y) = \vec q\lp( \vec y, \vec a \rp)$. 
% Since the largest coefficient in $\vec q$ is $\Omega_{d,m}(1)$ and each coordinate of $\vec a$ is bounded by $ O_d( \log(1/\delta) ) $, it follows that the largest coefficient in $\vec q_{\vec a}$ is at most $  \poly_{d,m}( \log(1/\delta) )$.
Next, define 
$f_{\vec a}': \R^m \mapsto \R$
as 
$f_{\vec a}'(\vec y) = f_{\vec a}\lp( \vec {\tilde \Sigma}(\vec y - \tilde {\vec \mu})  \rp) $.
Notice that 
$$
\poly_{d,m,N}( \log^{-1}(1/\delta) ) \; \delta^{d} \; \text{LC}(  f_{\vec a} )
\leq 
\text{LC}(  f_{\vec a}' )
\leq \poly_{d,m,N}( \log(1/\delta) ) \; \delta^{-d} \; \text{LC}(  f_{\vec a} ).
$$
Since $\E_{ \vec y \sim \normal( \vec 0, \vec I) }
\lp[
f_{\vec a}\lp( {\vec {\tilde \Sigma} }^{1/2} \lp(\vec y - \vec {\tilde \mu}\rp)\rp)
\rp]$ is $\Theta_{d,m}(1) \; \text{LC}(f_{\vec a}')$, the result follows.
\end{proof}

\begin{fact} \label{fact:lip-Gaussian-Density}
Let $\normal(\vec \mu, \vec \Sigma)$ be a distribution with
$\Sigma \geq \delta \vec I$.
Let $\vec x, \vec y$ be such that 
$ \snorm{2}{\vec x - \vec \mu}, \snorm{2}{\vec y - \vec \mu} \leq \delta^{-1/2} $
and
$ \snorm{2}{ \vec y - \vec x } \leq \delta^2 $
Then, it holds
$$
\Pr_{ \vec z \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ \vec z = \vec x  \rp]
= (1 \pm o(1)) 
\Pr_{ \vec z \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ \vec z = \vec y  \rp].
$$
\end{fact}
\begin{proof}
By direct computation, we have
$$
\frac{\Pr_{ \vec z \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ \vec z = \vec x  \rp] }{ \Pr_{ \vec z \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ \vec z = \vec y  \rp] }
= 
\exp \lp(  - 
\lp(\vec x - \vec \mu\rp)^T \Sigma^{-1} ( \vec x - \vec y ) +
\lp(\vec y - \vec \mu\rp)^T \Sigma^{-1} ( \vec x - \vec y ) -
\frac{1}{2} \; ( \vec x - \vec y )^T \Sigma^{-1} ( \vec x - \vec y )
 \rp).
$$
Since $\snorm{2}{ \vec \Sigma^{-1} } \leq \delta^{-1}$, $ \snorm{2}{\vec x - \vec \mu} \leq \delta^{-1/2},
\snorm{2}{\vec y - \vec \mu} \leq \delta^{-1/2}$ and $\snorm{2}{\vec x - \vec y} \leq \delta^2$, 
it follows that the terms in the exponents are all of order $o(1)$.
The fact then follows.
\end{proof}

\begin{claim}
\label{clm:near-uniform-gaussian-condition}
Let $\normal(\vec \mu, \vec \Sigma)$ be a $(\delta, N)$-reasonable Gaussian such that $ \log^N(1/\delta) < \delta^{-1/2}$.
Let $R \subset \R^m$ be an axis-aligned box defined as $ I_1 \times \cdots \times I_k \times \R^{m-k} $ where each $I_j$ is some interval that is at most $\delta^{-1/2}$-far from origin and of length at most $\delta^3$.
Denote $\bar R$ as $R$ restricted to the first $k$ dimensions: $\bar R = I_1 \times \cdots \times I_k$.
Then, for all $\vec q \in \bar R$
it holds
$$
\Pr_{\vec x \sim \normal(\vec \mu, \vec \Sigma)}
\lp[ \vec x_1 = \vec q_1, \cdots \vec x_k = \vec q_k | \vec x \in R \rp]
= (1 \pm o(1)) 
\frac{1}{ \text{vol}(\bar R) }.
$$
\end{claim}
\begin{proof}
% We claim that
% \begin{align} \label{eq:mixture-density-bounded-ratio}
% \Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
% \lp[  \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k | \vec x \in R \rp]
% = (1 \pm o(1)) \frac{1}{ \text{vol}(\bar R) }.    
% \end{align}
Notice that it suffices to show for any $\vec q, \vec q' \in R$, 
\begin{align}
\Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[  \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k  \rp]
= (1 \pm o(1)) 
\Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[  \vec x_1 = \vec q_1', \cdots, \vec x_k = \vec q_k' \rp].
\end{align}
Let $ \normal(\vec {\bar \mu}, \vec {\bar \Sigma})$ be the marginal distribution of 
$ \normal(\vec { \mu}, \vec { \Sigma})$ in the first $k$ coordinates.
It is easy to see we still have
$ \snorm{2}{ \vec {\bar \mu} } \leq 
\log^{N}(1/\delta) \leq \delta^{-1/2} $.
For $\vec {\bar \Sigma}$, since it is the principal sub-matrix of $\vec \Sigma$, we also have
$  \delta \vec I \leq \vec {\bar \Sigma} \leq \delta^{-1/2}  \vec I$.
Then, 
we note that $\Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[  \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k  \rp]$ is exactly 
$ \normal( \vec q; \vec {\bar \mu}, \vec {\bar \Sigma} ) $
and $\Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[  \vec x_1 = \vec q_1', \cdots, \vec x_k = \vec q_k'  \rp]$ is exactly 
$ \normal( \vec q'; \vec {\bar \mu}, \vec {\bar \Sigma} ) $.
Since $ \snorm{2}{ \vec q - \vec q' } \leq O_{d,m}( \delta^3 ) \leq \delta^2$, 
$ \snorm{2}{  \vec q - \vec {\bar \mu} }, \snorm{2}{ \vec q' - \vec {\bar \mu'} }  \leq 2 \; \delta^{-1/2}$, 
$  \vec {\bar \Sigma} \geq \delta \vec I $, we can use \Cref{fact:lip-Gaussian-Density} above and conclude the proof.
\end{proof}

\begin{lemma} \label{lem:average-individual-norm-ratio}
Let $d,m,N \in \mathbb Z^+$ and $\delta \in (0, 1/3)$ such that $ \log^N(1/\delta) < \delta^{-1/2}$.
Let $f: \R^m \mapsto \R$ be a degree-$d$ polynomial
and $\normal$ be a mixture of $(\delta, N)$-reasonable Gaussian distributions in $\R^m$.
Let $R \subset \R^m$ be an axis-aligned box defined as $ I_1 \times \cdots \times I_k \times \R^{m-k} $ where each $I_j$ is some interval that is at most $\delta^{-1/2}$-far from origin and of length at most $\delta^3$.
Then, for any $\normal(\vec \mu, \vec \Sigma)$ within the mixture, it holds
$$
\E_{ \vec x \sim \mathcal N }
\lp[ f^2(\vec x) | \vec x \in R
\rp]
\leq
\delta^{-3d}
% \poly_{d,m,N}( \log(1/\delta) ) \; \delta^{-2d}
\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x \in R
\rp].
$$
\end{lemma}
\begin{proof}
It suffices to argue that for two different Gaussians $\normal(\vec \mu, \vec \Sigma)$ and $\normal(\vec \mu', \vec \Sigma')$, the expectations of $f^2(\vec x)$  have bounded ratio:
$$
\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x \in R
\rp]
\leq 
\poly_{d,m}( \log(1/\delta) ) \; \delta^{-2d}
\E_{ \vec x \sim \normal(\vec \mu', \vec \Sigma') }
\lp[ f^2(\vec x) | \vec x \in R
\rp].
$$
Denote $\bar R$ as $R$ restricted to the first $k$ dimensions: $\bar R = I_1 \times \cdots \times I_k$.
For $\normal(\vec \mu, \vec \Sigma)$, we can rewrite the expectation as
\begin{align} \label{eq:conditional-expectation-norm}
&\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x \in R
\rp] \nonumber \\
&= 
\int_{ \vec q \in \bar R  }
\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k
\rp]
\Pr_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[  \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k | \vec x \in R \rp].    
\end{align}

By \Cref{clm:near-uniform-gaussian-condition}, we know that $\Pr_{ \vec x \sim \normal(\vec \mu, \Sigma) }
\lp[ \vec x_1 = \vec q_1 \cdots \vec x_k = \vec q_k \rp]$ is $1 \pm o(1)$ around the uniform distribution over $\bar R$. Combining this with \Cref{eq:conditional-expectation-norm}, we know it suffices to show that
\begin{align} \label{eq:same-q-condition-norm}
    &\E_{ \vec x \sim \normal(\vec \mu, \vec \Sigma) }
\lp[ f^2(\vec x) | \vec x_1 = \vec q_1, \cdots, \vec x_k \nonumber = \vec q_k
\rp] \nonumber \\
&\leq \poly_{d,m,N}(\log(1/\delta) ) \delta^{-2d}
\E_{ \vec x \sim \normal(\vec \mu', \vec \Sigma') }
\lp[ f^2(\vec x) | \vec x_1 = \vec q_1, \cdots, \vec x_k = \vec q_k
\rp].
\end{align}
for all $\vec q \in \bar R$.
Define $f_{\vec q}: \R^{m-k} \mapsto \R$ as
$  f_{\vec q}( \vec y  = f(\vec q, \vec y)) $.
By \Cref{eq:conditional-expectation-norm}, we can see both sides are within a factor of 
$\poly_{d,m,N}(\log(1/\delta) ) \delta^{-d}$ from 
the largest coefficient of $f_{\vec q}$.
Equation~\eqref{eq:same-q-condition-norm} then follows.
This concludes the proof of \Cref{lem:average-individual-norm-ratio}.
\end{proof}
